Interprocedural Dataflow Analysis over Weight Domains with Infinite Descending Chains

We study generalized fixed-point equations over idempotent semirings and provide an efficient algorithm for the detection whether a sequence of Kleene's iterations stabilizes after a finite number of steps. Previously known approaches considered only bounded semirings where there are no infinite descending chains. The main novelty of our work is that we deal with semirings without the boundedness restriction. Our study is motivated by several applications from interprocedural dataflow analysis. We demonstrate how the reachability problem for weighted pushdown automata can be reduced to solving equations in the framework mentioned above and we describe a few applications to demonstrate its usability.

==> correspondence-assertions.tex <==
\section{Correspondence Assertions and the Size-Change Termination Principle}
\label{app:ca}

In \cite{woo93semantic} Woo and Lam analyze protocols using the so-called
\emph{correspondences} between protocol points. A correspondence property
relates the occurrence of a transition to an earlier occurrence of some
other transition. In sequential programs (modelled as pushdown systems)
assume that assertions of
the form ${\tt begin}~\ell$ and ${\tt end}~\ell$ (where $\ell$ is a label
taken from a finite set of labels) are inserted by the programmer into
the code. The program is \emph{safe} if for each ${\tt end}~\ell$ reached at a
program point there is a unique corresponding ${\tt begin}~\ell$ at an
earlier execution point of the program.

Verifying safety via correspondence assertions can be done using
a similar technique as before. For each label $\ell$ we create
a weighted pushdown system based on the initially given boolean
program abstraction where every instruction ${\tt begin}~\ell$ has
the weight $+1$, every instruction ${\tt end}~\ell$ the weight $-1$,
and all other instructions have the weight $0$. Now the pushdown system
is safe if and only if
every reachable configuration has nonnegative accumulated weight.
This can be verified in polynomial time as outlined above.

Another application of our result seems to be
the size-change termination of programs~\cite{LeeJB01}. Similar
problems to ours are answered in order to prove
termination of first-order functional languages. As a part of our future work
we plan to take a closer look at this particular application.



==> dgraph.tex <==
\section{Dependency graph over an idempotent semiring}

\begin{definition}[Idempotent semiring] \label{def:semiring}
An \emph{idempotent semiring} is a 5-tuple
$\ring=(\domain, \combine, \extend, \combineNeutral, \extendNeutral)$
where $\domain$ is a set called the \emph{domain},
$\combineNeutral, \extendNeutral \in \domain$, and
the binary operators \emph{combine} `$\combine$'
and  \emph{extend} `$\extend$' on $\domain$ satisfy:
\begin{enumerate}
\item $(\domain, \combine)$ is a commutative monoid with $\combineNeutral$
as its neutral element and $(\domain, \extend)$ is a monoid
with $\extendNeutral$ as its neutral element,
\item extend distributes over combine, i.e.,
$\forall a, b, c \in \domain:
a \extend (b \combine c) = (a \extend b) \combine (a \extend c)$ and
$(a \combine b) \extend c = (a \extend c) \combine (b \extend c)$,
\item $\combineNeutral$ is an annihilator for extend, i.e.,
$\forall a \in \domain: a \extend \combineNeutral = \combineNeutral \extend a = \combineNeutral$, and
\item every $a \in \domain$ is idempotent w.r.t. combine, i.e., $\forall a \in \domain: a \combine a = a$.
%\item In the partial order $\sqsubseteq$ defined by
%  $\forall a, b \in \domain: a \sqsubseteq b ~\mbox{iff}~a \combine b = a$
%  there are no infinite descending chains.
\end{enumerate}
\end{definition}

\begin{definition}[Ordering and Bounded Width]\label{def:ordering}
We write $a \sqsubseteq b$ for $a,b \in \domain$ whenever $a \combine b = a$.
If the maximal number of incomparable elements w.r.t. $\sqsubseteq$
in the semiring $\ring$ is bounded by some constant $B$, we say
that the semiring is of \emph{bounded width} and the \emph{width} of $\ring$
is then the smallest such constant $B$.
%By $a \sqsubset b$ we mean $a \sqsubseteq b$ but $a \neq b$.
\end{definition}

\todo{JS: I have somewhere noted that we might also need that
if $a,b \not= \combineNeutral$ then $a \extend b \not= \combineNeutral$.
But now I cannot see why ... so this remark should be perhaps
discarded.}
As in this paper we are mainly interested in algorithmic approaches
to weighted pushdown automata, we shall implicitly
consider only \emph{computable} semirings
where the elements from the domain are enumerable,
operations combine and extend can be effectively computed and
the test on equality as well as $\sqsubseteq$ are decidable.
\todo{We should think more about the conditions on computable
semirings, this should be checked. This is just a sketch.}

\begin{lemma} \label{lem:properties}
(i) For all $a,b \in \domain$ holds that $a \combine b \sqsubseteq a$.
(ii) For all $a,b,c \in \domain$ holds that if
$a \sqsubseteq b$ then $a \extend c \sqsubseteq b \extend c$.

\end{lemma}
\begin{proof}
%Observe that $(a \combine b) \combine a = (a \combine a) \combine b =
%a \combine b$ due to associativity, commutativity and idempotency.
Straightforward.
\qed
\end{proof}

We shall now define an additional condition on the extend operator
that will be used later on in this section.

\begin{definition}
Given an idempotent semiring we say that \emph{extend preserves
inequality} if $a \not= b$ implies that $a \extend c \not= b \extend c$
for any $a, b, c \in (\domain \smallsetminus \{\combineNeutral\})$.
\end{definition}


\todo{Examples of semirings that will work for our algorithm, i.e., $\sqsubseteq$ is a total order and where extend preserves inequality.}
\begin{example} \label{ex:semirings}
The tuple $\ring_{\mathit int}
= (\integerswithinfty,\min,+,\infty,0)$ is an idempotent
semiring.
The domain are the integers extended
with infinity $\integerswithinfty = \integers \cup \set{\infty}$
where
$\min(\infty, a) = \min(a, \infty) = a$ and
$a + \infty = \infty + a = \infty$ for all $a \in \integerswithinfty$.
Combine is the minimum and extend is the usual addition on integers.
It is easy to see that $\ring_{\mathit int}$ meets
the requirements of Definition \ref{def:semiring}. It moreover preserves
inequality because the addition does and $\sqsubseteq$ is a total
ordering and hence the semiring is of width $1$.

Another example of an idempotent semirings is
$\ring_{\mathit rat}=(\rationals[0,1],\max,*,0,1)$
which is the semiring defined over the rationals in the interval from
$0$ to $1$. Here combine is the maximum and extend is the multiplication
on rationals.
This semiring $\ring_{\mathit rat}$ also meets the requirements of
Definition \ref{def:semiring}, preserves inequality and $\sqsubseteq$ is
a total ordering and hence the semiring is of width $1$.
\todo{add a remark on the product construction of a bounded width semiring with
a finite semiring, which gives again a bounded width semiring}
\qed
\end{example}

\begin{definition}[Dependency graph]
Let $\ring=(\domain,\combine,\extend,\combineNeutral,\extendNeutral)$
be an idempotent semiring. A \emph{dependency graph over $S$}
is a triple $G=(V,E,\tagged)$ where
$V$ is a finite set of \emph{nodes}, $E \subseteq V \times (\domain \cup V)
\times V$ is a finite set of \emph{edges} and $\tagged \subseteq V$ is
a set of \emph{tagged nodes}.
\end{definition}
We shall write $r \goes{x} r'$ whenever $(r,x,r') \in E$ and for technical
convenience (and without loss of generality) we
require that every node has at least
one incoming edge or it is a tagged node.

\begin{example} \label{ex:df}
Let $S_{\mathit{int}}
=(\integerswithinfty,\min,+,\infty,0)$ be the integer idempotent
semiring. Consider the following dependency graph over $S_{\mathit{int}}$.

\begin{center}
 \xymatrix@R=4ex@C=6ex{
 \nodedouble{r_1}
   \ar@/_1pc/[r]^{-2} \ar@/^3pc/[rrrrrrr]^{3}&
 \node{r_2} &
 \nodedouble{r_3}
   \ar@/_1pc/[r]^{1} \ar@/_2pc/[rr]^{-4}&
 \node{r_4} &
 \node{r_5}
   \ar@/_1.3pc/[ll]_{r_4} \ar@/_1pc/[r]^{r_8}&
 \node{r_6}
   \ar@/_1pc/[r]^{-4} \ar@/_2pc/[rr]^{1}&
 \node{r_7} &
 \node{r_8}
 }
\end{center}
The edges are labelled either by the elements from the domain of
the semiring, i.e. integers in our case, or by the names of other nodes in
the graph. By a double circle we denote the nodes that belong to
the set of tagged nodes, in our case $\tagged = \{r_1, r_3\}$. \qed
\todo{This is a dependency graph for the pushdown
$pX \definesto{3} pYY$, $pY \definesto{1} pYY$, $pY \definesto{-4} p$, $pX \definesto{-2} qX$.
It will be mentioned in the next section.}
\end{example}

For the rest of this section let us fix a dependency graph $G=(V,E,\tagged)$ over
$\ring=(\domain,\combine,\extend,\combineNeutral,\extendNeutral)$.
A valuation of the nodes in $G$ is a function
$\phi: V \rightarrow (\domain \cup \{\undefd\})$ which assigns to
every node a value from the domain $\domain$ or the undefined
value $\undefd$.

The intuition behind the dependency graph is that the edges show how
different nodes in the graph influence each other. This means that
if there is an edge $r \goes{d} r'$ in the graph such that $d \in
\domain$ then the value
$\phi(r')$ can be possibly improved by $\phi(r') :=
\phi(r') \combine (\phi(r)\extend d)$. If there is an edge
$r \goes{r''} r'$ such that $r'' \in V$ then the value of $\phi(r')$
can be possibly improved by $\phi(r') := \phi(r') \combine
(\phi(r) \extend \phi(r''))$. If the value $\phi(r')$ was improved
we say that the valuation $\phi$ was \emph{relaxed} along the given edge.


Assume now that we start with the initial valuation $\phi$ such
that $\phi(r) = \combineNeutral$ if $r \in V \smallsetminus \tagged$
and $\phi(r) = \extendNeutral$ if $r \in \tagged$. Observe that
by repeatedly relaxing $\phi$
along the edges in the dependency graph, the values in the nodes can either
stay stay unchanged or improve w.r.t. the ordering
relation $\sqsubseteq$ defined
in Definition~\ref{def:ordering} (because
$\phi(r') \combine (\phi(r) \extend d) \sqsubseteq \phi(r')$ and
$\phi(r') \combine (\phi(r) \extend \phi(r'')) \sqsubseteq \phi(r')$
due to Lemma~\ref{lem:properties} part (i)).
This means that either after a finite
number of relaxations we reach a unique
\todo{Check whether the fixed point is really unique!!!}
maximaaximall fixed point and no further relaxations
improve the current $\phi$, or the valuation $\phi$ improves
in some nodes infinitely often
(this can only happen if the relation $\sqsubseteq$
is not well founded). We shall argue that the latter situation can be
detected and in this case we will output the final $\phi$ which has the value
$\undefd$ assigned to all nodes that can be improved infinitely often.

\begin{example}
Consider the dependency graph from Example~\ref{ex:df}. We shall write
the valuation $\phi$ as a vector $(\phi(r_1), \phi(r_2), \ldots, \phi(r_8))$.
So initially we start with the valuation
$(0,\infty,0,\infty,\infty,\infty,\infty,\infty,\infty)$. Assume that
we relax once along every edge in the order which is determined by
$(r \goes{x} r') < (r'' \goes{x'} r''')$ iff
$r < r''$, or $r=r''$ and $r' < r'''$ where $r_1 < r_2 < \cdots < r_8$.
Hence after one round of eight relaxations we get the valuation
in the row labelled ``Round 1'', after a second round
we get the values in row labelled ``Round 2'' etc.
For example the value in ``Round 1'' for the node $r_3$ is $-3$
because by relaxing the edges $r_3 \goes{1} r_4$ and
$r_3 \goes{-4} r_5$ the nodes $r_4$ and $r_5$ get the values
$1$ and $-4$ respectively, and after relaxing along the edge
$r_5 \goes{r_4} r_3$ the node $r_3$ gets its value $-3=(-4)+1$.
\begin{center}
\begin{tabular}{c|lrcrcrcrcrcrcrcrcr}
Round &&
$r_1$ && $r_2$ && $r_3$ && $r_4$ && $r_5$ && $r_6$ && $r_7$ && $r_8$ &\\
\hline
0 & ( & 0 &,& $\infty$ &,& 0 &,& $\infty$ &,& $\infty$ &,& $\infty$
      &,& $\infty$ &,& $\infty$ &)\\
1 & ( & 0 &,& -2 &,& -3 &,& 1 &,& -4 &,& -1 &,& -5 &,& 0 &)\\
2 & ( & 0 &,& -2 &,& -9 &,& -2 &,& -7 &,& -7 &,& -11 &,& -6 &)\\
3 & ( & 0 &,& -2 &,& -21 &,& -8 &,& -13 &,& -19 &,& -23 &,& -18 &)\\
4 & ( & 0 &,& -2 &,& -45 &,& -20 &,& -25 &,& -43 &,& -47 &,& -46 &)\\
\vdots & ( & 0 &,& -2 &,& \vdots &,& \vdots &,& \vdots &,& \vdots &,&
  \vdots &,&  &)\\
\end{tabular}
\end{center}
It is clear that
the relaxation process never terminates and the valuation in the
nodes $r_3$ to $r_8$
will improve for ever. In this case we would like to detect this
situation and output the final valuation $(0, -2, \undefd,
\undefd, \undefd, \undefd, \undefd, \undefd)$. \qed
\end{example}

We shall now proceed to define formally the \emph{final valuation}
$\phi_f$ in the dependency graph $(V,E,\tagged)$.
First, we say that the pair $(r,d)$, where $r \in V$
is a node and $d \in \domain$ is an element from the domain, is
\emph{achievable} if there is a finite ordered proof
tree with its root labelled with $(r,d)$ such that
every node labelled with $(r',d')$ in the tree satisfies:
\begin{itemize}
\item if $(r',d')$ is a leaf then $r' \in \tagged$ and $d'=\extendNeutral$,
\item if $(r',d')$ is not a leaf then $(r',d')$ has either
\begin{itemize}
\item one child labelled with $(r_1,d_1)$ such that $r_1 \goes{d''} r'$
          with $d'' \in \domain$ and $d' = d_1 \extend d''$, or
\item one left child labelled with $(r_1,d_1)$ and one right child
      labelled with $(r_2,d_2)$ such that
      $r_1 \goes{r_2} r'$ and $d' = d_1 \extend d_2$.
\end{itemize}
\end{itemize}
The \emph{height} of the tree is the number of nodes on the longest
path from the root to some leaf. The intuition is that the proof tree
represents some possible order of relaxing the edges in the dependency
graph.

Now for every $r \in V$ we define its value $\phi_f(r)$ in the
\emph{final valuation} as follows:
$$ \phi_f(r) \defin
 \left\{
 \begin{array}{ll}
   \min\{ d \mid (r,d) \mbox{ is achievable } \} &
     \mbox{ if the minimum w.r.t. $\sqsubseteq$ exists } \\
   \undefd & \mbox{ otherwise.}
  \end{array}
  \right.
$$
Note that $\min \emptyset = \combineNeutral$.

\begin{example}
The tree bellow shows that in our running example the pair
$(r_8,-6)$ is achievable. For clarity reasons the edges to
single children are labelled by the weights of the corresponding
edges in the dependency graph.
\begin{center}
\mbox{
 \xymatrix@R=3ex@C=1ex{
 & & & (r_8,-6) \ar[d]_1 & & & \\
 & & & (r_6,-7) \ar[dll] \ar[drr] & & & \\
 & (r_5,-7) \ar[d]_{-4} & &  & & (r_8,0) \ar[d]_1 & \\
 & (r_3,-3) \ar[dl] \ar[dr] & & & & (r_6,-1) \ar[dl] \ar[dr] \\
 (r_5,-4) \ar[d]_{-4} & & (r_4,1)\ar[d]_1 & & (r_5,-4) \ar[d]_{-4} & &
  (r_8,3) \ar[d]_{3} \\
 (r_3,0) & & (r_3,0) & & (r_3,0) & & (r_1,0)
}}
\end{center}
The height of the tree is six and there are four paths that reach
the maximal length.
It is easy to see that the final valuation is $\phi_f=(0,-2,
\undefd, \undefd, \undefd, \undefd, \undefd, \undefd)$
because for the nodes from $r_3$ to $r_8$ there exist infinitely many
achievable pairs with
smaller and smaller values from the domain $\domain$.
 \qed
\end{example}

We shall now present a key lemma that, as shown later on,
guarantees a polynomial
running time for the computation of the final valuation $\phi_f$.

\begin{lemma} \label{lem:height}
Let $(V,E,\tagged)$ be a dependency graph over an idempotent semiring
$S$ of a bounded width $B$ %where $\sqsubseteq$ is a total ordering
and where extend preserves inequality. Let
$r \in V$ s.t. $\phi_f(r) \not= \undefd$. Then $(r,\phi_f(r))$
is achievable by a tree of height at most $|V|\cdot B$.
\end{lemma}
\begin{proof}
Let $\tagged_{\mathit min}$ by a tree of the minimal height for the achievable pair
$(r,\phi_f(r))$. If there are more trees of the minimal height,
we choose a $\tagged_{\mathit min}$
with minimal number of paths from the root to a leaf
that are of the maximal length.

Assume by contradiction that the height of $\tagged_{\mathit min}$
is more than $|V|\cdot B$ (the number of nodes in the dependency graph times
the width of the semiring).
Then necessarily for some $r' \in V$ there will be a path of the
maximal length from
the root to some leaf in $\tagged_{\mathit min}$ with two different nodes
labelled by
$(r',d_1)$ and $(r',d_2)$ such that the weights $d_1$ and $d_2$ are comparable.
This is because on such a path there will be some $r'$ occuring more thant
$B+1$ times and as the width of the semiring is $B$, at least two of the
corresponding weights have to be comparable.
%that $d_1 \sqsubseteq d_2$ or $d_2 \sqsubseteq d_1$.
Assume that the node labelled with $(r',d_1)$ is closer to the root
than $(r',d_2)$. We now have two possible cases.
% (due to the fact that $\sqsubseteq$ is a total ordering).
\begin{itemize}
\item
If $d_2 \sqsubseteq d_1$ then we remove the whole subtree rooted
by $(r',d_1)$ and replace it by the subtree rooted by $(r',d_2)$.
We also update the values in all pairs above $(r',d_2)$ accordingly.
Due to Lemma~\ref{lem:properties} part (ii) we know that in all
pairs above $(r',d_2)$ the values from the domain may only improve
w.r.t. $\sqsubseteq$ and surely the value in the root will remain
unchanged (if not we get a contradiction with the definition
of $\phi_f$). This means that the resulting tree remains
a proof tree for the achievable pair $(r,\phi_f(r))$, however, one of its
maximal paths is now shorter. This is a contradiction with the
choice of the minimal tree $\tagged_{\mathit min}$.
\item
If $d_1 \sqsubseteq d_2$ and $d_1 \not= d_2$
then let $\tagged_s$ be the subtree of $\tagged_{\mathit min}$ rooted
by $(r',d_1)$. Let us replace the subtree in $\tagged_{\mathit min}$
rooted by $(r',d_2)$
with $\tagged_s$ and update all the values in the pairs above $(r',d_1)$
accordingly. As $d_1$ is strictly bellow $d_2$ and because
extend preserves inequality we know that in combination with
Lemma~\ref{lem:properties} part (ii) all the values between
$(r',d_1)$ and the root of $\tagged_{\mathit min}$
will strictly improve w.r.t. $\sqsubseteq$.
Hence we have a tree which proves that $(r,d)$ is an achievable
pair and $d$ is strictly bellow $\phi_f(r)$. This
is a contradiction with the definition of $\phi_f(r)$.
\end{itemize}
\todo{perhaps add an illustration}
The lemma is hence proved.
\qed
\end{proof}

In Algorithm~\ref{alg:computation} we present
a pseudo-code for the computation of the final valuation of
a given dependency graph.

\begin{algorithm}[!ht]
\caption{Computation of the final valuation $\phi_f$}\label{alg:computation}
\begin{algorithmic}[1]
\REQUIRE A dependency graph $G=(V,E,\tagged)$ over an idempotent semiring
$\ring=(\domain, \combine, \extend, \combineNeutral, \extendNeutral)$
of bounded width $B$ %s.t. $\sqsubseteq$ is a total ordering and
where extend preserves inequality.
\ENSURE Final valuation $\phi:V \rightarrow (\domain \cup \{\undefd\})$.  \\
\STATE {\bf procedure} RELAX
\FOR {$i:= 1 \text{ to } |V|-1$}
 \FORALL {$(r,x,r') \in E$}
 \IF{$x \in \domain$}
 \STATE $\phi(r') := \phi(r') \combine (\phi(r) \extend x)$
 \ELSE[($x \in V$)]
 \STATE $\phi(r') := \phi(r') \combine (\phi(r) \extend \phi(x))$
 \ENDIF
 \ENDFOR
\ENDFOR
\STATE {\bf end}
\STATE
\STATE $\phi(r) := \combineNeutral$ for all $r \in V \smallsetminus \tagged$
\STATE $\phi(r) := \extendNeutral$ for all $r \in \tagged$
\STATE {\bf call} RELAX
\STATE $\phi_1 := \phi$
\STATE {\bf call} RELAX
\FORALL {$r \in V$}
\IF {$\phi_1(r) \not= \phi(r)$}
 \STATE $\phi(r) := \undefd$
\ENDIF
\ENDFOR
\RETURN $\phi$
\end{algorithmic}
\end{algorithm}


\begin{theorem} \label{thm:dg}
Algorithm~\ref{alg:computation} terminates and
outputs the final valuation $\phi_f$. Its running time is
$O_s(|V|\cdot |E|\cdot B)$ where $O_s$ denotes the asymptotic time complexity in
terms of the semiring operations, $(V,E,T)$ is the input dependency graph,
and $B$ is the width of the semiring.
 \todo{This $O_s$ notation should be
perhaps defined more precisely.}
\end{theorem}
\begin{proof}
Let us consider an achievable pair $(r,d)$ with a proof tree
of height $n$. By induction on $n$ we can easily establish
that after the main for-loop on lines 2--10 is executed $n-1$ times,
we get that $\phi(r) \sqsubseteq d$. The base case ($n=1$) is
obvious and the inductive step follows from Lemma~\ref{lem:properties}
part (ii). Now if $\phi_f(r) \not= \undefd$ we know that
there is an achievable pair $(r,\phi_f(r))$ with a proof tree
of height at most $|V|\cdot B$ (by Lemma~\ref{lem:height})
and hence after calling the procedure RELAX where
lines 2--10 are executed exactly $|V|\cdot B-1$ times,
we know that the final value for $r$
will be correctly computed by the algorithm. By calling the
procedure RELAX one more time we can observe in which nodes
there are still some improvements and these are then set
to $\undefd$ as they will improve for ever thanks to
Lemma~\ref{lem:properties} part (ii) and the fact that
extend preserves inequality.
\qed
\end{proof}

